Evolution of spiral galaxies in nonlocal gravity

We study the evolution of simulated disk galaxies in the context of a nonlocal theory of gravity. In this theory the appearance of the dark matter problem in cosmology and astrophysics is a manifestation of the nonlocality of the gravitational interaction. Using high-resolution N-body simulations, we investigate the dynamical evolution of disk galaxies and compare the result with the standard dark matter viewpoint. Specifically, we construct two exponential galaxy models, one in nonlocal gravity (NLG) and the other surrounded by a Plummer dark matter halo. Both systems start from the same baryonic matter distribution, particles velocities, random velocities and the initial Toomre's parameter. However, although the initial conditions are the same in both models, their long-term dynamics reveals some notable differences. For example, it turns out that the bar instability happens with higher rate in NLG model compared with the standard case. On the other hand, at the end of the simulation, we find that bars are weaker and faster in NLG compared with the standard case.

==> aliases.tex <==
\usepackage{xspace}

%  FORMATS
\newcommand{\dspaceon}{\renewcommand{\baselinestretch}{1.1}\large\normalsize}
\newcommand{\dspaceoff}{\renewcommand{\baselinestretch}{1}\large\normalsize}
\newcommand{\footon}{\dspaceoff\footnotesize}
\newcommand{\bk}{\!\!\!\!}

% MATH
\newcommand{\mean}[1]{\ensuremath{\langle#1\rangle}}
\newcommand{\abs}[1]{\lvert#1\rvert} 
\newcommand{\norm}[1]{\lVert#1\rVert}
\newcommand{\sub}[1]{\ensuremath{{_{\rm{#1}}}}}
\newcommand{\super}[1]{\ensuremath{{^{\rm{#1}}}}}
\newcommand{\rootn}{\ensuremath{\sqrt{n}}\xspace}

%  UNITS
\newcommand{\cps}{\,s$^{-1}$\xspace}
\newcommand{\un}[1]{\,\ensuremath{\rm{#1}}}
\newcommand{\as}{$^{\prime\prime}$\xspace}
\newcommand{\am}{$^{\prime}$\xspace}
\newcommand{\degrees}{$^{\circ}$}
\newcommand{\rsol}{\,$R_{\odot}$\xspace}
\newcommand{\lsol}{\,$L_{\odot}$\xspace}
\newcommand{\tsol}{\,$\tau_{\odot}$\xspace}
\newcommand{\msun}{\,$M_{\odot}$\xspace}
\newcommand{\msol}{\msun}
\newcommand{\lsun}{\,$L_{\odot}$\xspace}
\newcommand{\rsun}{\,$R_{\odot}$\xspace}
\newcommand{\msunperyear}{\msol\!$\rm yr^{-1}$\xspace}
\newcommand{\msolperyear}{\msunperyear}
\newcommand{\ergpersec}{\un{ergs\;s^{-1}}\xspace}
\newcommand{\ergpercmsec}{\un{ergs\,cm^{-2}\,s^{-1}}\xspace}
\newcommand{\percmsec}{\un{cm^{-2}\,s^{-1}}\xspace}
\newcommand{\percmsqrd}{\un{cm^{-2}}\xspace}
\newcommand{\phpercmseckev}{\un{ph\;cm^{-2}\,s^{-1}\,keV^{-1}}\xspace}
\newcommand{\phpercmsec}{\un{ph\;cm^{-2}\,s^{-1}}\xspace}
\newcommand{\rs}{\,$r_{\rm s}$\xspace}
\newcommand{\rlso}{\,$r_{\rm lso}$\xspace}
\newcommand{\rmso}{\,$r_{\rm mso}$\xspace}

%  INSTRUMENTS
\newcommand{\cgro}{{\em CGRO\/}\xspace}
\newcommand{\comptel}{{\small COMPTEL}\xspace}
\newcommand{\egret}{{\small EGRET}\xspace}
\newcommand{\integ}{{\sl INTEGRAL\/}\xspace}
\newcommand{\ibis}{{\small IBIS}\xspace}
\newcommand{\isgri}{{\small ISGRI}\xspace}
\newcommand{\picsit}{{\small PICSIT}\xspace}
\newcommand{\spi}{{\small SPI}\xspace}
\newcommand{\jemx}{{\small JEM-X}\xspace}
\newcommand{\omc}{{\small OMC}\xspace}
\newcommand{\hess}{{HESS}\xspace}

\newcommand{\fermi}{{\em Fermi}\xspace}
\newcommand{\uhuru}{{\em Uhuru}\xspace}
\newcommand{\ariel}{{\em Ariel\,V}\xspace}
\newcommand{\einstein}{{\em Einstein}\xspace}
\newcommand{\spacelab}{{\em Spacelab\,2}\xspace}
\newcommand{\xrt}{XRT\xspace}
\newcommand{\granat}{{\em Granat}\xspace}
\newcommand{\artp}{ART-P\xspace}
\newcommand{\sigm}{Sigma\xspace}
\newcommand{\ginga}{{\em Ginga}\xspace}
\newcommand{\asca}{{\em ASCA}\xspace}
\newcommand{\rosat}{{\em Rosat}\xspace}
\newcommand{\rxte}{{\small RXTE}\xspace}
\newcommand{\chandra}{{\em Chandra}\xspace}
\newcommand{\xmm}{{\em XMM-Newton}\xspace}
\newcommand{\suzaku}{{\em Suzaku}\xspace}
\newcommand{\epic}{{\small EPIC}\xspace}
\newcommand{\mos}{{\small MOS}\xspace}
\newcommand{\mosone}{{\small MOS1}\xspace}
\newcommand{\mostwo}{{\small MOS2}\xspace}
\newcommand{\pn}{{\small PN}\xspace}

\newcommand{\hst}{{\em HST\/}\xspace}
\newcommand{\hubble}{{\em Hubble Space Telescope\/}\xspace}
\newcommand{\keck}{{\it Keck}\xspace}
\newcommand{\cobe}{{\em COBE\/}\xspace}
\newcommand{\vla}{{\em VLA\/}\xspace}
\newcommand{\vlt}{{\em VLT\/}\xspace}


% SOURCES
\newcommand{\sgra}{Sgr\,A$^{*}$\xspace}
\newcommand{\sgraeast}{Sgr\,A\;East\xspace}
\newcommand{\sgrawest}{Sgr\;A\;West\xspace}
\newcommand{\igr}{IGR\,J17456--2901\xspace}
\newcommand{\ax}{AX\,J17456--2901\xspace}
\newcommand{\cxogc}{CXOGC\,J174540.0--290031\xspace}
\newcommand{\cxo}{\cxogc}
\newcommand{\xmmu}{XMMU\,J174554.4--285456\xspace}
\newcommand{\eg}{3EG\,J1746--2851\xspace}
\newcommand{\hessgc}{HESS\,J1745--290\xspace}


% WORDS
\newcommand{\afterTwoYears}{{\em A Persistent High-Energy Flux from the Heart of the Milky Way: INTEGRAL's View of the Galactic Center\/}\xspace}
\newcommand{\gammarays}{$\gamma$-rays\xspace}
\newcommand{\gammaray}{$\gamma$-ray\xspace}
\newcommand{\xray}{X-ray\xspace}
\newcommand{\xrays}{X-rays\xspace}
\newcommand{\fwhm}{FWHM\xspace}
\newcommand{\gti}{{\small GTI}\xspace}
\newcommand{\gtis}{{\small GTI}s\xspace}
\newcommand{\psla}{{\small PSLA}\xspace}
\newcommand{\arf}{{\small ARF}\xspace}
\newcommand{\arfs}{{\small ARF}s\xspace}
\newcommand{\rmf}{{\small RMF}\xspace}
\newcommand{\rmfs}{{\small RMF}s\xspace}
\newcommand{\pwn}{{\small PWN}\xspace}
\newcommand{\sn}{{\small SN}\xspace}
\newcommand{\snr}{{\small SNR}\xspace}
\newcommand{\snrs}{{\small SNR}s\xspace}
\newcommand{\gc}{{\small GC}\xspace}
\newcommand{\gcde}{{\small GCDE}\xspace}
\newcommand{\gd}{Galactic disk\xspace}
\newcommand{\gn}{{\small GN}\xspace}
\newcommand{\psf}{{\small PSF}\xspace}
\newcommand{\spsf}{{\small SPSF}\xspace}
\newcommand{\rms}{{\small RMS}\xspace}
\newcommand{\go}{{\small GO}\xspace}
\newcommand{\xspec}{{\small XSPEC}\xspace}
\newcommand{\glimpse}{{\small GLIMPSE}\xspace}
\newcommand{\ir}{{\small IR}\xspace}
\newcommand{\nir}{near-\ir}
\newcommand{\uv}{{\small UV}\xspace}
\newcommand{\ic}{{\small IC}\xspace}
\newcommand{\bh}{{\small BH}\xspace}
\newcommand{\osa}{{\small OSA}\xspace}
\newcommand{\sas}{{\small SAS}\xspace}
\newcommand{\isdc}{{\small ISDC}\xspace}
\newcommand{\ccd}{{\small CCD}\xspace}
\newcommand{\ccds}{{\small CCD}s\xspace}
\newcommand{\lmxb}{{\small LMXB}\xspace}
\newcommand{\lmxbs}{{\small LMXB}s\xspace}
\newcommand{\ism}{{\small ISM}\xspace}
\newcommand{\gmc}{{\small GMC}\xspace}
\newcommand{\gmcs}{{\small GMC}s\xspace}
\newcommand{\cmz}{{\small CMZ}\xspace}
\newcommand{\cnd}{{\small CND}\xspace}
\newcommand{\imf}{{\small IMF}\xspace}
\newcommand{\ura}{URA\xspace}
\newcommand{\mura}{MURA\xspace}
\newcommand{\og}{OG\xspace}
\newcommand{\ssc}{SSC\xspace}
\newcommand{\lso}{LSO\xspace}
\newcommand{\mso}{MSO\xspace}
\newcommand{\xrb}{XRB\xspace}
\newcommand{\xrbs}{XRBs\xspace}
\newcommand{\pdf}{{\small PDF\/}\xspace}
\newcommand{\cdf}{{\small CDF\/}\xspace}
\newcommand{\dof}{{\small DOF\/}\xspace}
\newcommand{\dft}{{\small DFT\/}\xspace}
\newcommand{\fft}{{\small FFT\/}\xspace}
\newcommand{\ifs}{{\small IFS\/}\xspace}
\newcommand{\psd}{{\small PSD\/}\xspace}
\newcommand{\pds}{{\small PDS\/}\xspace}


\newcommand{\hone}{H\,{\sc i\/}\xspace}
\newcommand{\htwo}{H\,{\sc ii\/}\xspace}
\newcommand{\neontwo}{Ne\,{\sc ii\/}\xspace}
\newcommand{\feone}{Fe\,{\sc i\/}\xspace}
\newcommand{\fetwentyfive}{Fe\,{\sc xxv\/}\xspace}
\newcommand{\fetwentysix}{Fe\,{\sc xxvi\/}\xspace}
\newcommand{\nione}{Ni\,{\sc i\/}\xspace}
\newcommand{\nitwentyseven}{Ni\,{\sc xxvii\/}\xspace}

